Arithmetic Multivariate Descartes' Rule

Let L be any number field or $\mathfrak{p}$-adic field and consider F:=(f_1,...,f_k) where f_i is in L[x_1,...,x_n]\{0} for all i and there are exactly m distinct exponent vectors appearing in f_1,...,f_k. We prove that F has no more than 1+(cmn(m-1)^2 log m)^n geometrically isolated roots in L^n, where c is an explicit and effectively computable constant depending only on L. This gives a significantly sharper arithmetic analogue of Khovanski's Theorem on Fewnomials and a higher-dimensional generalization of an earlier result of Hendrik W. Lenstra, Jr. for the case of a single univariate polynomial. We also present some further refinements of our new bounds and briefly discuss the complexity of finding isolated rational roots.

==> amdmaple <==
# J. Maurice Rojas, Oct. 31, 2001
# Happy Halloween!
# 
# Last update: Nov. 15, 2001 
#

Digits:=40; 
c:=exp(1)/(exp(1)-1) ; 
f:= m-> 6*8*c^2*(1+log(2/log(2))/log(2))*(m-1)*m*(1+log((m-1)/log(2))/log(2)); 
g:= m-> 4*4*c^2*(m+1)^4*(1+log((m+1)/log(2))/log(2))^2; 
h:= m-> 4*(2^m-2) ; 

# f is the bound from corollary 1, applied to example 1. 
# g is the bound from theorem 1, applied to example 1. 
# h is the real analytic bound mentioned in example 1.
# asymptotically, f<g<h, but this doesn't really kick  
#  in until after a certain point...

# f finally starts beating g at m=3...
printf("Corollary 1 beats Theorem 1 (but not Real Analytic) already at m=3:\n cor1 = %d , thm1 = %d , realanalytic = %d\n\n",floor(f(3)/2),floor(g(3)),floor(h(3))); 

# not to mention m=4...
printf("...not to mention m=4:\n cor1 = %d , thm1 = %d , realanalytic = %d\n\n",floor(f(4)),floor(g(4)),floor(h(4))); 


# f finally starts beating h at m=17...
printf("Corollary 1 finally starts beating Real Analytic at m=17:\n cor1 = %d , realanalytic = %d\n\n",floor(f(17)),floor(h(17))) ; 

# g doesn't start beating h until m=29...
printf("Theorem 1 doesn't start beating Real Analytic until m=29:\n thm1 = %d , realanalytic = %d\n\n", floor(g(29)) , floor(h(29))) ; 


